MMViR: A Multi-Modal and Multi-Granularity Representation for Long-range Video Understanding

Long videos, ranging from minutes to hours, present significant challenges for current Multi-modal Large Language Models (MLLMs) due to their complex events, diverse scenes, and long-range dependencies. Direct encoding of such videos is computationally too expensive, while simple video-to-text conversion often results in redundant or fragmented content. To address these limitations, we introduce MMViR, a novel multi-modal, multi-grained structured representation for long video understanding. MMViR identifies key turning points to segment the video and constructs a three-level description that couples global narratives with fine-grained visual details. This design supports efficient query-based retrieval and generalizes well across various scenarios. Extensive evaluations across three tasks, including QA, summarization, and retrieval, show that MMViR outperforms the prior strongest method, achieving a 19.67% improvement in hour-long video understanding while reducing processing latency to 45.4% of the original.

==> table2.tex <==
\begin{table*}[h!]
\centering
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{p{4.0cm} p{2.5cm} p{4.0cm} p{5.2cm}}
\toprule
\textbf{Question} & \textbf{Task} & \textbf{Answer} & \textbf{Justification} \\
\midrule
In the process of securing the laptop's bottom access panel, did the camera wearer use the screwdriver or the bolts more frequently? & reasoning: 
Temporal frequency & Both were used with the same frequency. & The frames show bolts and a screwdriver \textbf{\textcolor{blue}{being used in coordination to secure the bottom access panel}}, indicating both were utilized with the same frequency. \\
\hline
What item did the camera wearer use to secure components during the hardware tasks? & perception:

factual\_recall & Screwdriver & The close-up frames show the camera wearer securing components using a screwdriver, \textbf{\textcolor{blue}{which is visible in their right hand in multiple instances}}. \\
\hline
Summarize the key interactions and events in the video, focusing on their impact and significance. & summarization: key\_events & The camera wearer and Person A collaborate in the kitchen, with a playful start and they share cooking tips, emphasizing teamwork and the educational aspect of cooking. & The playful start \textbf{\textcolor{blue}{is evident from the casual teamwork, and the conclusion highlights a friendly dynamic emphasizing teamwork}} and the social aspect of cooking, as suggested by the interactions seen in the sampled frames. \\
\hline
Select the correct statement about spatial relationships depicted in the video. & reasoning: 
spatial relationship & The cooker is located in the front left of the dining table. & The cooker is stationed near the front left of the dining table \textbf{\textcolor{blue}{as visible in frames 4, 9, and 10}}, where the table and cooker share the same vicinity. \\
\bottomrule
\end{tabular}
\caption{Case analysis of the answers and their justification for VideoQA under the Hourvideo Dataset, the blue-highlighted parts indicate the reasons behind the generated answer.}
\label{tab:case}
\end{table*}
